VasTSD: Learning 3D Vascular Tree-state Space Diffusion Model for Angiography Synthesis

Angiography imaging is a medical imaging technique that enhances the visibility of blood vessels within the body by using contrast agents. Angiographic images can effectively assist in the diagnosis of vascular diseases. However, contrast agents may bring extra radiation exposure which is harmful to patients with health risks. To mitigate these concerns, in this paper, we aim to automatically generate angiography from non-angiographic inputs, by leveraging and enhancing the inherent physical properties of vascular structures. Previous methods relying on 2D slice-based angiography synthesis struggle with maintaining continuity in 3D vascular structures and exhibit limited effectiveness across different imaging modalities. We propose VasTSD, a 3D vascular tree-state space diffusion model to synthesize angiography from 3D non-angiographic volumes, with a novel state space serialization approach that dynamically constructs vascular tree topologies, integrating these with a diffusion-based generative model to ensure the generation of anatomically continuous vasculature in 3D volumes. A pre-trained vision embedder is employed to construct vascular state space representations, enabling consistent modeling of vascular structures across multiple modalities. Extensive experiments on various angiographic datasets demonstrate the superiority of VasTSD over prior works, achieving enhanced continuity of blood vessels in synthesized angiographic synthesis for multiple modalities and anatomical regions.

==> sec/algorithm.tex <==
% \begin{algorithm}[htbp]
% \caption{Tree Scanning Algorithm}
% \label{alg:tree_scanning}
% \begin{algorithmic}[1]
% \REQUIRE Input feature map $X = \{x_i\}_{i=1}^L$
% \ENSURE Output feature map $output$

% \STATE $L \gets \text{length}(X)$
% \STATE $m \gets 4$ if \text{isImageTask} else $3$
% \STATE $G \gets \text{initializeGraph}(V, E)$

% \FOR{$i = 1$ \TO $L$}
%     \FOR{$j \in \text{getNeighbors}(i, m)$}
%         \STATE $weight \gets \text{computeCosineDistance}(X[i], X[j])$
%         \STATE $\text{addEdge}(G, i, j, weight)$
%     \ENDFOR
% \ENDFOR

% \STATE $G_T \gets \text{kruskalMST}(G)$
% \FOR{each node $i$ in $G_T$}
%     \STATE $h[i] \gets 0$
% \ENDFOR

% \FOR{each node $i$ in $\text{postOrderTraversal}(G_T)$}
%     \FOR{each neighbor $j$ in $\text{getNeighbors}(i)$}
%         \STATE $h[i] \gets h[i] + S(E[i, j]) \cdot B[j] \cdot X[j]$
%     \ENDFOR
% \ENDFOR

% \FOR{each node $i$ in $\text{preOrderTraversal}(G_T)$}
%     \STATE $\text{propagateState}(i, h[i])$
% \ENDFOR

% \STATE $output \gets C \cdot (A \cdot h + D \cdot X)$
% \RETURN $output$
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[htbp]
% \caption{Tree Scanning Algorithm}
% \label{alg:tree_scanning}
% \begin{algorithmic}[1]
% \REQUIRE Input feature map $X = \{x_i\}_{i=1}^L$, Target feature map $Y$
% \ENSURE Output feature map $output$, Gradients $\left\{ \frac{\partial \text{Loss}}{\partial X}, \frac{\partial \text{Loss}}{\partial B}, \frac{\partial \text{Loss}}{\partial A}, \frac{\partial \text{Loss}}{\partial C} \right\}$

% \STATE $L \gets \text{length}(X)$; $m \gets 4$
% \STATE $G \gets \text{initializeGraph}(V, E)$

% \FOR{$i = 1$ \TO $L$}
%     \FOR{$j \in \text{getNeighbors}(i, m)$}
%         \STATE $weight \gets \text{computeCosineDistance}(X[i], X[j])$
%         \STATE $\text{addEdge}(G, i, j, weight)$
%     \ENDFOR
% \ENDFOR

% \STATE $G_T \gets \text{kruskalMST}(G)$
% \FOR{each node $i$ in $G_T$}
%     \STATE $h[i] \gets 0$
% \ENDFOR

% \FOR{each node $i$ in $\text{postOrderTraversal}(G_T)$}
%     \FOR{each neighbor $j$ in $\text{getNeighbors}(i)$}
%         \STATE $h[i] \gets h[i] + S(E[i, j]) \cdot B[j] \cdot X[j]$
%     \ENDFOR
% \ENDFOR

% \FOR{each node $i$ in $\text{preOrderTraversal}(G_T)$}
%     \STATE $\text{propagateState}(i, h[i])$
% \ENDFOR

% \STATE $output \gets C \cdot (A \cdot h + D \cdot X)$

% % Loss Calculation
% \STATE $\text{Loss} \gets \text{loss\_function}(output, Y)$

% % Backward Propagation: Compute gradients
% \STATE Compute $\frac{\partial \text{Loss}}{\partial \text{output}}$
% \STATE Backpropagate through tree to compute $\frac{\partial \text{Loss}}{\partial h}$
% \FOR{each node $i$ in $G_T$}
%     \STATE Compute $\frac{\partial \text{Loss}}{\partial X[i]}$, $\frac{\partial \text{Loss}}{\partial B[i]}$, $\frac{\partial \text{Loss}}{\partial A[i]}$, and $\frac{\partial \text{Loss}}{\partial C}$
% \ENDFOR

% \RETURN $output$, $\left\{ \frac{\partial \text{Loss}}{\partial X}, \frac{\partial \text{Loss}}{\partial B}, \frac{\partial \text{Loss}}{\partial A}, \frac{\partial \text{Loss}}{\partial C} \right\}$
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[htbp]
% \caption{Tree Scanning Algorithm}
% \label{alg:tree_scanning}
% \begin{algorithmic}[1]
% \REQUIRE Input feature map $X = \{x_i\}_{i=1}^L$, Target feature map $Y$
% \ENSURE Output feature map $output$, Gradients $\left\{ \frac{\partial \text{Loss}}{\partial X}, \frac{\partial \text{Loss}}{\partial B}, \frac{\partial \text{Loss}}{\partial A}, \frac{\partial \text{Loss}}{\partial C} \right\}$

% \STATE $L \gets \text{length}(X)$, $m \gets 4$
% \STATE $G \gets \text{initializeGraph}(V, E)$

% \FOR{$i = 1$ \TO $L$}
%     \FOR{$j \in \text{getNeighbors}(i, m)$}
%         \STATE $w \gets \text{computeCosineDistance}(X[i], X[j])$
%         \STATE $\text{addEdge}(G, i, j, w)$
%     \ENDFOR
% \ENDFOR

% \STATE $G_T \gets \text{kruskalMST}(G)$
% \FOR{each node $i$ in $G_T$}
%     \STATE $h[i] \gets 0$
% \ENDFOR

% \FOR{each node $i$ in $\text{postOrderTraversal}(G_T)$}
%     \STATE $h[i] \gets \sum_{j \in \text{getNeighbors}(i)} S(E[i,j]) \cdot B[j] \cdot X[j]$
% \ENDFOR

% \FOR{each node $i$ in $\text{preOrderTraversal}(G_T)$}
%     \STATE $\text{propagateState}(i, h[i])$
% \ENDFOR

% \STATE $output \gets C \cdot (A \cdot h + D \cdot X)$

% % Loss Calculation and Backpropagation
% \STATE Compute initial gradient $\eta_i = \frac{\partial \text{Loss}}{\partial h_i}$

% % Aggregation Phase: Update gradients from leaf to root
% \FOR{each node $i$ in $\text{postOrderTraversal}(G_T)$}
%     \STATE $\eta_i \gets \bar{B}_i \cdot \frac{\partial \text{Loss}}{\partial h_i} + \sum_{j \in \{ t \mid \text{Par}(t) = i \}} \eta_j \cdot \bar{A}_j$
% \ENDFOR

% % State Propagation Phase: Propagate gradients from root to leaf
% \FOR{each node $i$ in $\text{preOrderTraversal}(G_T)$}
%     \STATE $\eta_i \gets \bar{A}_i \cdot \eta_i$
%     \FOR{each child node $j$ of $i$}
%         \STATE $\eta_j \gets \bar{B}_j \cdot \eta_i$
%     \ENDFOR
% \ENDFOR

% % Tree Scan Loss Calculation
% \STATE $\mathcal{L}_{\text{scan}} \gets \sum_{i} \frac{1}{2} \| \eta_i \|^2$

% % Compute gradients with respect to parameters
% \FOR{each node $i$ in $G_T$}
%     \STATE Compute $\frac{\partial \text{Loss}}{\partial X[i]}, \frac{\partial \text{Loss}}{\partial B[i]}, \frac{\partial \text{Loss}}{\partial A[i]}, \frac{\partial \text{Loss}}{\partial C}$
% \ENDFOR

% \RETURN $output$, gradients
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[htbp]
% \caption{Tree Scanning Algorithm}
% \label{alg:tree_scanning}
% \begin{algorithmic}[1]
% \REQUIRE Input feature map $X = \{x_i\}_{i=1}^L$, Target feature map $Y$
% \ENSURE Output feature map $output$, Gradients $\left\{ \frac{\partial \text{Loss}}{\partial X}, \frac{\partial \text{Loss}}{\partial B}, \frac{\partial \text{Loss}}{\partial A}, \frac{\partial \text{Loss}}{\partial C} \right\}$

% \STATE $L \gets \text{length}(X)$; $m \gets 4$
% \STATE $G \gets \text{initializeGraph}(V, E)$

% \FOR{$i = 1$ \TO $L$}
%     \FOR{$j \in \text{getNeighbors}(i, m)$}
%         \STATE $weight \gets \text{computeCosineDistance}(X[i], X[j])$
%         \STATE $\text{addEdge}(G, i, j, weight)$
%     \ENDFOR
% \ENDFOR

% \STATE $G_T \gets \text{kruskalMST}(G)$
% \FOR{each node $i$ in $G_T$}
%     \STATE $h[i] \gets 0$
% \ENDFOR

% \FOR{each node $i$ in $\text{postOrderTraversal}(G_T)$}
%     \FOR{each neighbor $j$ in $\text{getNeighbors}(i)$}
%         \STATE $h[i] \gets h[i] + S(E[i, j]) \cdot B[j] \cdot X[j]$
%     \ENDFOR
% \ENDFOR

% \FOR{each node $i$ in $\text{preOrderTraversal}(G_T)$}
%     \STATE $\text{propagateState}(i, h[i])$
% \ENDFOR

% \STATE $output \gets C \cdot (A \cdot h + D \cdot X)$

% % Loss Calculation
% \STATE $\text{Loss} \gets \text{loss\_function}(output, Y)$

% % Backward Propagation: Compute gradients
% \STATE Compute $\frac{\partial \text{Loss}}{\partial \text{output}}$
% \STATE Backpropagate through tree to compute $\frac{\partial \text{Loss}}{\partial h}$
% \FOR{each node $i$ in $G_T$}
%     \STATE Compute $\frac{\partial \text{Loss}}{\partial X[i]}$, $\frac{\partial \text{Loss}}{\partial B[i]}$, $\frac{\partial \text{Loss}}{\partial A[i]}$, and $\frac{\partial \text{Loss}}{\partial C}$
% \ENDFOR

% \RETURN $output$, $\left\{ \frac{\partial \text{Loss}}{\partial X}, \frac{\partial \text{Loss}}{\partial B}, \frac{\partial \text{Loss}}{\partial A}, \frac{\partial \text{Loss}}{\partial C} \right\}$
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[htbp]
\caption{Vascular Tree Scanning Algorithm}
\label{alg:tree_scanning}
\begin{algorithmic}[1]
\REQUIRE Input feature map $X = \{x_i\}_{i=1}^L$, Target $Y$
\ENSURE Output feature map $output$, Gradients $\left\{ \frac{\partial \text{Loss}}{\partial X}, \frac{\partial \text{Loss}}{\partial B}, \frac{\partial \text{Loss}}{\partial A}, \frac{\partial \text{Loss}}{\partial C} \right\}$

\STATE $G \gets \text{initializeGraph}(V, E)$
\FOR{$i = 1$ \TO $L$} \FOR{$j \in \text{getNeighbors}(i, 4)$} \STATE $\text{addEdge}(G, i, j, \text{computeCosineDistance}(X[i], X[j]))$ \ENDFOR \ENDFOR
\STATE $G_T \gets \text{kruskalMST}(G)$, $h[i] \gets 0 \ \forall i \in G_T$

\FOR{each node $i$ in $\text{postOrderTraversal}(G_T)$}
    \STATE $h[i] \gets \sum_{j \in \text{getNeighbors}(i)} S(E[i,j]) \cdot B[j] \cdot X[j]$
\ENDFOR

\FOR{each node $i$ in $\text{preOrderTraversal}(G_T)$} \STATE $\text{propagateState}(i, h[i])$ \ENDFOR

\STATE $output \gets C \cdot (A \cdot h + D \cdot X)$

% Backpropagation
\STATE $\eta_i \gets \frac{\partial \text{Loss}}{\partial h_i}$

\FOR{each node $i$ in $\text{postOrderTraversal}(G_T)$}
    \STATE $\eta_i \gets \bar{B}_i \cdot \eta_i + \sum_{j \in \{ t \mid \text{Par}(t) = i \}} \eta_j \cdot \bar{A}_j$
\ENDFOR

\FOR{each node $i$ in $\text{preOrderTraversal}(G_T)$}
    \STATE $\eta_i \gets \bar{A}_i \cdot \eta_i$, $\eta_j \gets \bar{B}_j \cdot \eta_i$ for each child $j$
\ENDFOR

\STATE $\mathcal{L}_{\text{scan}} \gets \sum_{i} \frac{1}{2} \| \eta_i \|^2$

% Gradients w.r.t. parameters
\FOR{each node $i$ in $G_T$} \STATE Compute gradients for $X[i], B[i], A[i], C$ \ENDFOR

\RETURN $output$, gradients
\end{algorithmic}
\end{algorithm}



% \begin{algorithm}[htbp]
% \caption{Vascular Tree Scanning Algorithm}
% \label{alg:tree_scanning}
% \begin{algorithmic}[1]
% \REQUIRE $X = \{x_i\}_{i=1}^L$, $Y$
% \ENSURE $output$, gradients

% \STATE $G \gets \text{initializeGraph}(V, E)$, $G_T \gets \text{kruskalMST}(G)$, $h[i] = 0, \forall i \in G_T$
% \FOR{$i = 1$ \TO $L$} 
%     \FOR{$j \in \text{getNeighbors}(i, 4)$} 
%         \STATE $\text{addEdge}(G, i, j, \text{cosineDist}(X[i], X[j]))$ 
%     \ENDFOR
% \ENDFOR
% % \STATE $h[i] = \sum_{j \in \text{Neigh}(i)} S(E[i,j]) \cdot B[j] \cdot X[j], \forall i \in G_T$
% \STATE $h[i] = \sum_{j \in \text{Neigh}(i)} S(E[i,j]) \cdot B[j] \cdot X[j], \forall i \in G_T$
% \STATE $output = C \cdot (A \cdot h + D \cdot X), \eta_i \gets \frac{\partial \mathcal{L}}{\partial h_i}$
% % \STATE $\eta_i \gets \frac{\partial \mathcal{L}}{\partial h_i}, \quad \forall i \in G_T$
% \FOR{$i \in G_T$ (Bottom-up \& Top-down)}
%     \STATE $\eta_i \gets \bar{B}_i \eta_i + \sum_{j \in \text{Children}(i)} \eta_j \bar{A}_j$
%     \STATE $\eta_j \gets \bar{B}_j \eta_i, \quad \forall j \in \text{Children}(i)$
% \ENDFOR
% \STATE $\mathcal{L}_{\text{scan}} = \sum_{i} \frac{1}{2} \| \eta_i \|^2$
% \RETURN $output$, gradients
% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[htbp]
% \caption{Vascular Tree Scanning Algorithm}
% \label{alg:tree_scanning}
% \begin{algorithmic}[1]
% \REQUIRE $X = \{x_i\}_{i=1}^L$, $Y$
% \ENSURE $output$, gradients

% \STATE $G \gets \text{initializeGraph}(V, E)$, $G_T \gets \text{kruskalMST}(G)$, $h[i] = 0, \forall i \in G_T$
% \FOR{$i = 1$ \TO $L$} 
%     \FOR{$j \in \text{getNeighbors}(i, 4)$} 
%         \STATE $\text{addEdge}(G, i, j, \text{cosineDist}(X[i], X[j]))$ 
%     \ENDFOR
% \ENDFOR
% \STATE $h[i] = \sum_{j \in \text{Neigh}(i)} S(E[i,j]) \cdot B[j] \cdot X[j], \forall i \in G_T$
% \STATE $output = C \cdot (A \cdot h + D \cdot X), \eta_i \gets \frac{\partial \mathcal{L}}{\partial h_i}$
% \FOR{$i \in G_T$ \text{(Bottom-up \& Top-down)}}
%     \STATE $\eta_i \gets \bar{B}_i \eta_i + \sum_{j \in \text{Children}(i)} \eta_j \bar{A}_j$
%     \STATE $\eta_j \gets \bar{B}_j \eta_i, \quad \forall j \in \text{Children}(i)$
% \ENDFOR
% \STATE $\mathcal{L}_{\text{scan}} = \sum_{i} \frac{1}{2} \| \eta_i \|^2$
% \RETURN $output$, gradients
% \end{algorithmic}
% \end{algorithm}

==> tables/result1.tex <==
\begin{table*}[]
\centering
% \resizebox{\linewidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc}
\hline
\multirow{3}{*}{Methods} & \multicolumn{6}{c|}{ITKTubeTK}                                                                                                                       & \multicolumn{2}{c}{Topcow2024}              \\ \cline{2-9} 
                        & \multicolumn{2}{c|}{T1-Flash} & \multicolumn{2}{c|}{T2} & \multicolumn{2}{c|}{T1-Mprage} & \multicolumn{2}{c}{CTA} \\ \cline{2-9} 
                        & \centering PSNR         & SSIM                              & PSNR      & SSIM                              & PSNR                    & SSIM                     & PSNR                 & SSIM                 \\ \hline
SAGAN~\cite{zhang2019self}                   & 27.85        & 0.9184                            & 28.16     & 0.9254                            & 27.96                   & 0.9234                   & 25.32                & 0.9018               \\
cGAN~\cite{dar2019image}
& 28.45        & 0.9248                            & 28.73     & 0.9289                            & 28.68                   & 0.9264                   & 25.58                & 0.9142               \\ \hline
SynDiff~\cite{ozbey2023unsupervised}
& 28.98        & \underline{0.9446}                            & 29.06     & \textbf{0.9482}                            & 29.12                   & \textbf{0.9516}                   & 26.13                & \underline{0.9317}               \\
Fast-DDPM~\cite{jiang2024fast}               & 26.92        & 0.8958                            & 27.51     & 0.9024                            & 27.37                   & 0.8984                   & 24.15                & 0.8924               \\ 
DiffMa~\cite{wang2024soft}                  & \underline{29.12}        & 0.6936                            & \underline{29.36}     & 0.7174                            & \underline{29.28}                   & 0.7058                   & \underline{26.76}                & 0.7286               \\ \hline
VasTSD                 & \textbf{29.86}        & \textbf{0.9478}                            & \textbf{29.72}     & \underline{0.9384}                            & \textbf{29.92}                   & \underline{0.9454}                   & \textbf{27.36}                & \textbf{0.9372}               \\ \hline
\end{tabular}
\caption{\textbf{Comparison of modal conversion methods for synthesizing MRA from 2D Slices.} PSNR (dB) $\uparrow$ and SSIM $\uparrow$ results across the test set. The best and the second-best results are highlighted in \textbf{bold} and \underline{underline}.}
\label{tab:result_tran}
\end{table*}


==> tables/result2.tex <==
% \begin{table}[ht]
% \centering
% \caption{\textbf{Comparison....} PSNR (dB) $\uparrow$ and SSIM $\uparrow$ results across the test set. The best and the second-best results are highlighted in \textbf{bold} and \underline{underline}.}
% \label{tab:result_cta}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{c|c|c|c|c|c|c}
% \hline
%      & SAGAN  & cGAN   & SynDiff & Fast-DDPM & DiffMa & VasTSD \\ \hline
% PSNR & 26.42  & 27.87  & 28.56   & 27.38     & 28.94  & 29.48  \\ \hline
% SSIM & 0.8921 & 0.9163 & 0.9321  & 0.9128    & 0.9428 & 0.9562 \\ \hline
% \end{tabular}}
% \end{table}

